AmodalSynthDrive: A Synthetic Amodal Perception Dataset for Autonomous Driving

Unlike humans, who can effortlessly estimate the entirety of objects even when partially occluded, modern computer vision algorithms still find this aspect extremely challenging. Leveraging this amodal perception for autonomous driving remains largely untapped due to the lack of suitable datasets. The curation of these datasets is primarily hindered by significant annotation costs and mitigating annotator subjectivity in accurately labeling occluded regions. To address these limitations, we introduce AmodalSynthDrive, a synthetic multi-task multi-modal amodal perception dataset. The dataset provides multi-view camera images, 3D bounding boxes, LiDAR data, and odometry for 150 driving sequences with over 1M object annotations in diverse traffic, weather, and lighting conditions. AmodalSynthDrive supports multiple amodal scene understanding tasks including the introduced amodal depth estimation for enhanced spatial understanding. We evaluate several baselines for each of these tasks to illustrate the challenges and set up public benchmarking servers. The dataset is available at http://amodalsynthdrive.cs.uni-freiburg.de.

==> sections/datasetsTable.tex <==

%\newcommand*{\chk}[1][]{\tikz[x=1em, y=1em]\fill[#1] (0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}
\newcommand*{\chk}[1][]{\tikz[x=1em, y=1em]\fill[#1] (0,.35) -- (.25,0) -- (1,.7) -- (.25,.2) -- cycle;}
\newcommand{\STAB}[2][c]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand*{\vertical}[1]{\rotatebox[origin=c]{90}{#1}}
\newcommand*{\vertical}[1]{\begin{sideways}{#1}\end{sideways}}
\newcommand*{\ua}{\textbf{*}}
%\newcommand*{\vertical}[2][c]{\STAB[#1]{\rotatebox[origin=c]{90}{#2}}}
%\newcommand*{\vertical}[2][c]{\rotatebox[origin=c]{90}{\parbox[#1]{#2}}}
\newcommand{\colgrpspace}{1em}
\newcommand{\cmidrulespace}{1.5em}


\begin{table*}[ht]
    \centering
    \captionsetup{width=.70\linewidth}
    \caption{Comparison of different medical datasets, grouped by the scope of inputs. \change{Datasets marked as \emph{Real} were recorded from actual surgeries, while \emph{Simulated} were enacted on cadavers or dummies. Computer-generated data is marked as \emph{Synthetic}.} The data from datasets marked with \ua{} was neither publicly available nor easily accessible at the time of this writing.}
    \label{tab:datasets}
    
    \footnotesize
    \begin{tabular}{clcc<{\hspace{\colgrpspace}}ccc<{\hspace{\colgrpspace}}cc<{\hspace{\colgrpspace}}cccr}
    %\begin{tabular}{cl@{\hskip 3em}cc@{\hskip 3em}ccc@{\hskip 3em}cc@{\hskip 3em}cccr}
    \toprule
    & & \multicolumn{9}{c}{Task / Annotations} &  \\
    \cmidrule(lr){3-11}
    & & & & \multicolumn{3}{c<{\hspace{\colgrpspace}}}{Segmentation} & \multicolumn{2}{c<{\hspace{\colgrpspace}}}{Depth} & & & & \multirow{2}{*}[-5.3em]{\makecell{Annotated\\Samples}}\\
    \cmidrule(lr{\cmidrulespace}){5-7} \cmidrule(lr{\cmidrulespace}){8-9}
    & Dataset & \vertical{Classification} & \vertical{Detection} & \vertical{Instance} & \vertical{Semantic} & \vertical{Panoptic} & \vertical{Monocular} & \vertical{Stereo} & \vertical{Human Pose} & \vertical{Scene Graph} & Type \\
    \midrule
    
    \multirow{4}{*}{\vertical{MIS}}%                    | cls  | det  | inst | sem  | pan  | mono | ster | pose | scen | type      | samples
    & Cholect50~\cite{nwoye2022cholect50}               & \chk &  --  &  --  & --   & --   & --   & --   &  --  &  --  & Real      & \num{100863} \\
    & DSAD~\cite{carstens2023dsad}                      & \chk &  --  & --   & \chk & --   & --   & --   &  --  &  --  & Real      & \num{ 14625} \\
    & AutoLaparo~\cite{wang2022autolaparo}              & \chk &  --  & \chk & --   & --   & --   & --   &  --  &  --  & Real      & \num{  1800} \\
    & HeiCo~\cite{maier2021heico}                       & \chk &  --  & \chk & --   & --   & --   & --   &  --  &  --  & Real      & \num{ 10040} \\
    %& Ex-vivo dVRK~\cite{colleoni2020exvivo}            &      &  --  &      & \chk & --   & --   & --   &  --  &  --  & Simulated & \num{  4200} \\
    
    \midrule
    
    \multirow{3}{*}{\vertical{\makecell{Open\\Surgery}}}%           | cls  | det  | inst | sem  | pan  | mono | ster | pose | scen | type      | samples
    & CATARACTS~\cite{al2019cataracts}                  & \chk &  --  & --   &  --  & --   & --   & --   &  --  & --   & Real      & \num{957884} \\
    & Surgical Tools~\cite{fujii2022surgicaltools}\ua{} & --   & \chk & --   &  --  & --   & --   & --   &  --  & --   & Real      & \num{ 19560} \\
    %& StereotacticScene~\cite{li2022brain}\ua{}         & --   & \chk & --   & \chk & --   & --   & --   &  --  & --   & Real      & \num{  1578} \\
    & CaDIS~\cite{grammatikopoulou2021cadis}            & --   &  --  & --   & \chk & --   & --   & --   &  --  & --   & Real      & \num{  4670} \\
    %& HOSPI-Tools~\cite{rodrigues2022hospitools}        & --   & \chk & --   & \chk & --   & --   & --   &  --  & --   & Simulated & \num{ 15522} \\
    
    \midrule
    
    \multirow{6}{*}[-0.5em]{\vertical{General OR}}%             | cls  | det  | inst | sem  | pan  | mono | ster | pose | scen | type      | samples
    & Auto OR~\cite{sharghi2020autoor}\ua{}             & \chk &  --  &  --  & --   &  --  &  --  & --   & --   &  --  & Real      & N/A \\
    & MVOR~\cite{srivastav2021mvor}                     & --   & \chk &  --  & --   &  --  & \chk & --   & \chk &  --  & Real      & \num{   732} \\
    & Robotic3DOR~\cite{li2020orenvaware}\ua{}          & --   &  --  &  --  & \chk &  --  &  --  & --   &  --  &  --  & Simulated & \num{  7980} \\
    & MultiHumanOR~\cite{belagiannis2016skeletons}      & --   &  --  &  --  & --   &  --  &  --  & --   & \chk &  --  & Simulated & \num{   700} \\
    & 4D-OR~\cite{oszoy20224dor}                        & --   & \change{--} &  --  & --   &  --  & \chk & \chk & \chk & \chk & Simulated & \num{  6780} \\
    \cmidrule{2-13}
    & \textbf{\datasetname{} (Ours)}                    & --   & \chk & \chk & \chk & \chk & \chk &  --  & --   &  --  & Synthetic & \num{48000} \\
    
    \bottomrule
\end{tabular}
\end{table*}

% \begin{table*}
% \centering
% \caption{Comparison between publicly available medical datasets, grouped by the scope of the inputs.}
% \label{tab:datasets}

% \footnotesize
% \begin{tabular}{clccccccccccccr}

% \toprule
% & & \multicolumn{9}{c}{Task / Annotations} & \multicolumn{3}{c}{Type} \\
% \cmidrule(lr){3-11} \cmidrule(lr){12-14}
% & & & & \multicolumn{3}{c}{Segmentation} & \multicolumn{2}{c}{Depth} \\
% \cmidrule(lr){5-7} \cmidrule(lr){8-9}
% & Dataset & \vertical{Classification} & \vertical{Detection} & \vertical{Instance} & \vertical{Semantic} & \vertical{Panoptic} & \vertical{Monocular} & \vertical{Stereo} & \vertical{Human Pose} & \vertical{Scene Graph} & \vertical{Real} & \vertical{Simulated} & \vertical{Synthetic} & \makecell{Annotated\\Samples}\\
% \midrule

% \multirow{5}{*}{\vertical{MIS}}%               | cls  | det  | inst | sem  | pan  | mono | ster | pose | scen | real | sim  | synt | samples
% & Cholect50~\cite{nwoye2022cholect50}          & \chk &      &      &      &      &      &      &      &      & \chk &      &      & \num{100863} \\
% & DSAD~\cite{carstens2023dsad}                 & \chk &      &      & \chk &      &      &      &      &      & \chk &      &      & \num{ 14625} \\
% & AutoLaparo~\cite{wang2022autolaparo}         & \chk &      & \chk &      &      &      &      &      &      & \chk &      &      & \num{  1800} \\
% & HeiCo~\cite{maier2021heico}                  & \chk &      & \chk &      &      &      &      &      &      & \chk &      &      & \num{ 10040} \\
% & Ex-vivo dVRK~\cite{colleoni2020exvivo}       &      &      &      & \chk &      &      &      &      &      &      & \chk &      & \num{  4200} \\

% \midrule

% \multirow{5}{*}{\vertical{Open Surgery}}%      | cls  | det  | inst | sem  | pan  | mono | ster | pose | scen | real | sim  | synt | samples
% & CATARACTS~\cite{al2019cataracts}             & \chk &      &      &      &      &      &      &      &      & \chk &      &      & \num{957884} \\
% & Surgical Tools~\cite{fujii2022surgicaltools} &      & \chk &      &      &      &      &      &      &      & \chk &      &      & \num{ 19560} \\
% & StereotacticScene~\cite{li2022brain}         &      & \chk &      & \chk &      &      &      &      &      & \chk &      &      & \num{  1578} \\
% & CaDIS~\cite{grammatikopoulou2021cadis}       &      &      &      & \chk &      &      &      &      &      & \chk &      &      & \num{  4670} \\
% & HOSPI-Tools~\cite{rodrigues2022hospitools}   &      & \chk &      & \chk &      &      &      &      &      &      & \chk &      & \num{ 15522} \\

% \midrule

% \multirow{6}{*}{\vertical{General OR}}%        | cls  | det  | inst | sem  | pan  | mono | ster | pose | scen | real | sim  | synt | samples
% & Auto OR~\cite{sharghi2020autoor}             & \chk &      &      &      &      &      &      &      &      & \chk &      &      & \red{?} \\
% & MVOR~\cite{srivastav2021mvor}                &      & \chk &      &      &      & \chk &      & \chk &      & \chk &      &      & \num{   732} \\
% & Robotic3DOR~\cite{li2020orenvaware}     &      &      &      & \chk &      &      &      &      &      &      & \chk &      & \num{  7980} \\
% & MultiHumanOR~\cite{belagiannis2016skeletons} &      &      &      &      &      &      &      & \chk &      &      & \chk &      & \num{   700} \\
% & 4D-OR~\cite{oszoy20224dor}                   &      & \chk &      &      &      & \chk & \chk & \chk & \chk &      & \chk &      & \num{  6780} \\
% \cmidrule{2-15}
% & \textbf{\datasetname{} (Ours)}               &      & \chk & \chk & \chk & \chk & \chk &  &      &      &      &      & \chk & \num{ 16000} \\
% \bottomrule
% \end{tabular}
% \vspace{-0.2cm}
% \end{table*}


